Two Unicast Information Flows over Linear Deterministic Networks

We investigate the two unicast flow problem over layered linear deterministic networks with arbitrary number of nodes. When the minimum cut value between each source-destination pair is constrained to be 1, it is obvious that the triangular rate region {(R_1,R_2):R_1,R_2> 0, R_1+R_2< 1} can be achieved, and that one cannot achieve beyond the square rate region {(R_1,R_2):R_1,R_2> 0, R_1< 1,R_2< 1}. Analogous to the work by Wang and Shroff for wired networks, we provide the necessary and sufficient conditions for the capacity region to be the triangular region and the necessary and sufficient conditions for it to be the square region. Moreover, we completely characterize the capacity region and conclude that there are exactly three more possible capacity regions of this class of networks, in contrast to the result in wired networks where only the triangular and square rate regions are possible. Our achievability scheme is based on linear coding over an extension field with at most four nodes performing special linear coding operations, namely interference neutralization and zero forcing, while all other nodes perform random linear coding.

==> Prelim.tex <==
A node is \emph{$\msf{s}_i$-reachable} if it can be reached by $\msf{s}_i$. It is \emph{$\msf{s}_i$-only-reachable} if it can be reached by $\msf{s}_i$ but not $\msf{s}_j$, $j\ne i$. It is \emph{$\msf{s}_1\msf{s}_2$-reachable} if it can be reached by both $\msf{s}_1$ and $\msf{s}_2$. 

For each node $\msf{v}\in\mcal{V}\setminus\{\msf{s}_1,\msf{s}_2\},$
\begin{itemize}
\item let $\mcal{P}^{\msf{s}_i}(\msf{v})\subseteq \mcal{P}(\msf{v})$ denote the set of parents of $\msf{v}$ \emph{reachable} by source $\msf{s}_i$, $i=1,2,$
\item let $\mcal{K}(\msf{v}):=\lbp \msf{u}: \mcal{P}(\msf{u}) = \mcal{P}(\msf{v})\rbp$ denote the \emph{clones} of $\msf{v},$ the set of nodes that receive the same signal as $\msf{v},$ 
\item let $\mcal{K}^{\msf{s}_i}(\msf{v}):=\lbp \msf{u}: \mcal{P}^{\msf{s}_i}(\msf{u}) = \mcal{P}^{\msf{s}_i}(\msf{v})\rbp, i=1,2,$ the set of nodes that have the same $\msf{s}_i$-reachable parents as $\msf{v}.$
\end{itemize}

The following table illustrates these sets of nodes for the node $\msf{u}_4$ in the two example networks in Fig.~\ref{fig_examples}.
%\begin{center}
%{\small
%\begin{tabular}{|c|c|c|c|c|c|c|c| }
%  \hline
%  & Fig.~\ref{fig_examples}(a) & Fig.~\ref{fig_examples}(b) & & Fig.~\ref{fig_examples}(a) & Fig.~\ref{fig_examples}(b) \\ \hline
%  $\mcal{P}(\msf{u}_4)$ & $\{\msf{u}_1,\msf{u}_2\}$ & $\{\msf{u}_1,\msf{u}_2\}$ & $\mcal{K}(\msf{u}_4)$ & $\{\msf{u}_4\}$ & $\{\msf{u}_4\}$ \\ \hline
%  $\mcal{P}^{\msf{s}_1}(\msf{u}_4)$ & $\{\msf{u}_1,\msf{u}_2\}$ & $\{\msf{u}_1\}$ & $\mcal{K}^{\msf{s}_1}(\msf{u}_4)$ & $\{\msf{u}_4\}$ & $\{\msf{u}_4,\msf{u}_6\}$ \\ \hline
%  $\mcal{P}^{\msf{s}_2}(\msf{u}_4)$ & $\{\msf{u}_2\}$ & $\{\msf{u}_2\}$ & $\mcal{K}^{\msf{s}_2}(\msf{u}_4)$ & $\{\msf{u}_3,\msf{u}_4\}$ & $\{\msf{u}_4,\msf{u}_5\}$ \\ \hline
%%  $\mcal{K}(\msf{u}_4)$ & $\{\msf{u}_4\}$ & $\{\msf{u}_4\}$ \\ \hline
%%  $\mcal{K}^{\msf{s}_1}(\msf{u}_4)$ & $\{\msf{u}_4\}$ & $\{\msf{u}_4,\msf{u}_6\}$ \\ \hline
%%  $\mcal{K}^{\msf{s}_2}(\msf{u}_4)$ & $\{\msf{u}_3,\msf{u}_4\}$ & $\{\msf{u}_4,\msf{u}_5\}$ \\ \hline
%\end{tabular}
%}
%\end{center}
\begin{center}
{\small
\begin{tabular}{|c|c|c|c|c|c|c|c| }
  \hline
  & Fig.~\ref{fig_examples}(a) & Fig.~\ref{fig_examples}(b) \\ \hline
  $\mcal{P}(\msf{u}_4)$ & $\{\msf{u}_1,\msf{u}_2\}$ & $\{\msf{u}_1,\msf{u}_2\}$ \\ \hline
  $\mcal{P}^{\msf{s}_1}(\msf{u}_4)$ & $\{\msf{u}_1,\msf{u}_2\}$ & $\{\msf{u}_1\}$ \\ \hline
  $\mcal{P}^{\msf{s}_2}(\msf{u}_4)$ & $\{\msf{u}_2\}$ & $\{\msf{u}_2\}$ \\ \hline
  $\mcal{K}(\msf{u}_4)$ & $\{\msf{u}_4\}$ & $\{\msf{u}_4\}$ \\ \hline
  $\mcal{K}^{\msf{s}_1}(\msf{u}_4)$ & $\{\msf{u}_4\}$ & $\{\msf{u}_4,\msf{u}_6\}$ \\ \hline
  $\mcal{K}^{\msf{s}_2}(\msf{u}_4)$ & $\{\msf{u}_3,\msf{u}_4\}$ & $\{\msf{u}_4,\msf{u}_5\}$ \\ \hline
\end{tabular}
}
\end{center}

For two sets of nodes $\mcal{U}_1$ and $\mcal{U}_2$, we say a collection of nodes $\mcal{T}$ is a $(\mcal{U}_1;\mcal{U}_2)$-vertex-cut if in the graph obtained from the deletion of $\mcal{T},$ there are no paths from any node in $\mcal{U}_1\setminus \mcal{T}$ to any node in $\mcal{U}_2\setminus\mcal{T}.$ Note that this definition allows $\mcal{T}$ to have nodes from $\mcal{U}_1$ or $\mcal{U}_2.$

We say a node $\msf{v}\in\mcal{V}$ is \emph{omniscient} if it satisfies either of (A) or (B) below:
\begin{itemize}
{\rm
\item[(A)] $\mcal{K}(\msf{v})$ is a $\lp\msf{s}_1,\msf{s}_2; \msf{d}_1\rp$-vertex-cut and $\mcal{K}^{\msf{s}_2}(\msf{v})$ is a $\lp \msf{s}_2; \msf{d}_2\rp$-vertex-cut.% \emph{OR}
\item[(B)] $\mcal{K}(\msf{v})$ is a $\lp\msf{s}_1,\msf{s}_2; \msf{d}_2\rp$-vertex-cut and $\mcal{K}^{\msf{s}_1}(\msf{v})$ is a $\lp \msf{s}_1; \msf{d}_1\rp$-vertex-cut.
}
\end{itemize}

